SGD and Hogwild! Convergence Without the Bounded Gradients Assumption

Stochastic gradient descent (SGD) is the optimization algorithm of choice in many machine learning applications such as regularized empirical risk minimization and training deep neural networks. The classical convergence analysis of SGD is carried out under the assumption that the norm of the stochastic gradient is uniformly bounded. While this might hold for some loss functions, it is always violated for cases where the objective function is strongly convex. In (Bottou et al.,2016), a new analysis of convergence of SGD is performed under the assumption that stochastic gradients are bounded with respect to the true gradient norm. Here we show that for stochastic problems arising in machine learning such bound always holds; and we also propose an alternative convergence analysis of SGD with diminishing learning rate regime, which results in more relaxed conditions than those in (Bottou et al.,2016). We then move on the asynchronous parallel setting, and prove convergence of Hogwild! algorithm in the same regime, obtaining the first convergence results for this method in the case of diminished learning rate.

==> Fixed_stepsize.tex <==
\subsection{Fixed stepsize}
\label{subsec:hogwild_fixedstepsize}

We consider a processor $P$ make an inconsistent read $\hat{w}_t$ of $w$  at the moment $t-\rho_t$ (i.e., $w=w_{t-\rho_t}$) and updates $w$ at the moment $t$ ($w=w_t$) with an amount of $-\eta_t \langle \nabla f(\hat{w}_t;\xi_t),e[s_t] \rangle e[s_t]$. The convergence of the sequence $\hat{w}_t$ is guaranteed if $\eta_t \leq \frac{\alpha_t\Delta}{\mu(t+E)}$ with $4 \leq \alpha_t \leq \alpha$. Assume that $t-\rho_t+E \in [2^h,2^{h+1}]$ for a certain $h$. Then, the stepsize $\eta_t$ can be fixed as $\frac{4}{\mu 2^h}$ for all $t$ such as $t-\rho_t+E \in [2^h,2^{h+1}]$. 
%and the sequence $w^t$ still converges because $\eta_t = \frac{2}{\mu 2^h} < \frac{\alpha_t}{\mu(t+E)} < \frac{\alpha}{\mu(t+E)}$. 
The reason is as follows. Since $E \geq 2R \geq 2\rho_t$ (see Assumption~\ref{Assumption:hogwild_rhot}), $\rho_t \leq t+E-\rho_t$. Therefore, $t+E=t+E-\rho_t + \rho_t \leq 2(t+E-\rho_t)$. This inequality combines with the given fact $t+E-\rho_t \leq 2^{h+1}$ yields $$t+E \leq 2^{h+2}.$$

This implies $\frac{4(t+E)}{2^h}\leq 16$. Let choose $\alpha_t \geq \frac{4(t+E)}{2^h}$ and $\alpha=16$. Since $t+E \geq t+E -\rho_t \geq 2^h$, $$\alpha_t \geq 4.$$  

Moreover, $\frac{4}{2^h} \leq \frac{\alpha_t}{t+E} \leq \frac{\alpha}{t+E}$. In other words, $\eta_t = \frac{4}{\mu 2^h} \leq \frac{\alpha_t}{\mu (t+E)} \leq \frac{\alpha}{\mu(t+E)}$. The convergence rate of the algorithm with this fixed stepsize in each period $[2^h,2^{h+1}]$ follows Theorem~\ref{theorem:Hogwild_newnew1}.

\begin{algorithm}[h!]
   \caption{Hogwild! with fixed stepsize}
   \label{algo:hogwild_fixed_stepsize}
\begin{algorithmic}
  \STATE $t \leftarrow 1$, $h \leftarrow \log_2(E)$
  \STATE Compute $\eta = \frac{4}{\mu 2^h}$
     \STATE Let Hogwild! algorithms runs
  \FOR{$t=1,2\dotsc$} 
    \STATE Increasing $t=t+1$ when a processor updates $w$ with stepsize $\eta$
    \STATE If $t+E>2^{h+1}$, then $\eta=\eta/2$ and $h=h+1$
  \ENDFOR  
\end{algorithmic}
\end{algorithm}

We describes Hogwild! with fixed stepsize in Algorithm~\ref{algo:hogwild_fixed_stepsize} for a given $E$ and $\mu$. It is worthy to highlight that SGD is a special case of the algorithm of Hogwild! described in this paper. It implies that Algorithm~\ref{algo:hogwild_fixed_stepsize} works pretty well for SGD case. Thus, we now know when and how we should diminish the stepsize to make $\hat{w}_t$ (or $w_t$) converge. 

In the previous section, we prove the convergence of Hogwild! for the diminishing stepsize $\eta_t$. In the algorithm, $\eta_t$ is required to change for every update of the shared solution $w$ and it is not so practical. Thus, Algorithm~\ref{algo:hogwild_fixed_stepsize} makes the Hogwild! with the diminishing stepsize being practical now because the user does not need to tune the stepsize for every step. It is obvious that, when $h$ is sufficient large enough, the gap between $2^h$ and $2^{h+1}$ is very large. Thus, even we have some wrong updates of variable $t$ and $h$ when the locking mechanism is not used for these variables, the convergence of $w$ is not affected. This is the most importance of Algorithm~\ref{algo:hogwild_fixed_stepsize}, i.e., the user does not to tune the stepsize or the stepsize is automatically decaying. 



 
